Contribution of solar hydrogen Ly{\alpha} line emission in total ionization rate in ionospheric D-region during the maximum of solar X-flare

The solar Ly{\alpha} line emission can be considered as the dominant source of ionization processes in the ionospheric D-region at altitudes above 70 km during unperturbed conditions. However, large sudden impacts of radiation in some other energy domains can also significantly influence the ionization rate and, in this paper, we present a study on the contribution of Ly {\alpha} radiation to the ionization rate when the ionosphere is disturbed by solar X-flares. We give relevant analytical expressions and make calculations and numerical simulations for the low ionosphere using data collected by the VLF receiver located in Serbia for the VLF radio signal emitted by the DHO transmitter in Germany.

==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.8em{\hfil.\hfil}%
\setbox8=\hbox to0.8em{\hfil$^{#1}$\hfil}%
\box7\kern-0.8em\box8}}

\def\dd{\point{\rm d}}
\def\hh{\point{\rm h}}
\def\mm{\point{\rm m}}
\def\ss{\point{\rm s}}

\def\oo{\point{\circ}}
\def\lll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



